Toric codes and quantum doubles from two-body Hamiltonians

We present a procedure to obtain the Hamiltonians of the toric code and Kitaev quantum double models as the low-energy limits of entirely two-body Hamiltonians. Our construction makes use of a new type of perturbation gadget based on error-detecting subsystem codes. The procedure is motivated by a PEPS description of the target models, and reproduces the target models' behavior using only couplings which are natural in terms of the original Hamiltonians. This allows our construction to exactly capture the symmetries of the target models.

==> Sections/conclusion.tex <==
% This line sets the project root file.
% 
% !TEX root = ../main.tex
% 
%------------------------------------------------------------------------------------------------------------%


%------------------------------------------------------------------------------------------------------------%
\section{Conclusion}\label{S:conc}
%------------------------------------------------------------------------------------------------------------%

Our results describe a new perturbative method for obtaining the quantum double models as the effective low-energy behaviour of a two-body Hamiltonian. This is done with only linear overhead in qubits with the system size. The code gadget Hamiltonians and perturbation terms we use are closely related to the original models on simple surfaces, and in this sense our approach uses only natural couplings. As such, our treatment may be amenable to experimental realization similarly to the Kitaev honeycomb model. Our construction also preserves the symmetries of the original models exactly. 

Perturbative corrections which remain within the codespace of our construction will not have significant effect on the ground space of the model (at reasonable orders), as our method exploits the algebra of the quantum double models themselves to prohibit unwanted terms from arising. However it is an open question as to the effect of perturbative corrections which can leave the codespace (though these are heavily suppressed by energy penalty).


